Disentangling Speakers in Multi-Talker Speech Recognition with Speaker-Aware CTC

Multi-talker speech recognition (MTASR) faces unique challenges in disentangling and transcribing overlapping speech. To address these challenges, this paper investigates the role of Connectionist Temporal Classification (CTC) in speaker disentanglement when incorporated with Serialized Output Training (SOT) for MTASR. Our visualization reveals that CTC guides the encoder to represent different speakers in distinct temporal regions of acoustic embeddings. Leveraging this insight, we propose a novel Speaker-Aware CTC (SACTC) training objective, based on the Bayes risk CTC framework. SACTC is a tailored CTC variant for multi-talker scenarios, it explicitly models speaker disentanglement by constraining the encoder to represent different speakers' tokens at specific time frames. When integrated with SOT, the SOT-SACTC model consistently outperforms standard SOT-CTC across various degrees of speech overlap. Specifically, we observe relative word error rate reductions of 10% overall and 15% on low-overlap speech. This work represents an initial exploration of CTC-based enhancements for MTASR tasks, offering a new perspective on speaker disentanglement in multi-talker speech recognition. The code is available at https://github.com/kjw11/Speaker-Aware-CTC.

==> tables/t1.tex <==

\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\vspace{-10pt}
\centering

\caption{
WER (\%) of vanilla CTC in MTASR. "dec." stands for decoding.
}
\vspace{-8pt}
\label{tab:t1}
\scalebox{0.8}{
\renewcommand{\arraystretch}{1.3} % line hight
\begin{tabular}{l|l|cc|cc|cccc}
\bottomrule

\multirow{3}{*}{\textbf{ID}} & \makecell[c]{\multirow{3}{*}{
\textbf{System}}}  &\multicolumn{2}{c|}{\textbf{Librispeech}} &\multicolumn{6}{c}{\textbf{LibrispeechMix-2mix}} \\
 \cline{3-4} \cline{5-10} 
& & \multirow{2}{*}{\textbf{dev}} & \multirow{2}{*}{\textbf{test}} & \multirow{2}{*}{\textbf{Dev}} & \multirow{2}{*}{\shortstack{\textbf{Test}\\(Overall)}}& \multicolumn{4}{c}{\textbf{Test} (Conditional)} \\
\cline{7-10}
% & & & & & & \textbf{(0, 20]} & \textbf{(20, 50]} & \textbf{(50, 100]} & \textbf{Average} \\
& & & & & & low & mid & high & OA-WER \\
% & & & & & & low & median & high & OA-WER \\
\noalign{\hrule height 0.9pt}
A1 & SOT & 4.1 & 4.6 & 8.1 & 9.2 & 9.0 & \hl{8.0} & \hl{12.8} & 9.9 \\
\hline
B1 & CTC & 5.0 & 5.4 & 11.7 & 11.1 & 7.5 & 12.4 & 18.2 & 12.7\\
\hline
C1 & SOT+CTC & 4.3 & \hl{4.5} & 8.4  & \hl{8.8} & \hl{7.1} & 9.0  & 13.1 & \hl{9.7}\\
C2 & \, $\hookrightarrow$ AED only dec. & 4.8 & 5.4 & 11.5 & 12.9 & 11.7 & 12.5 & 17.3& 13.8\\
C3 & \, $\hookrightarrow$ CTC only dec. & 5.5 & 5.6 & 12.7 & 12.0 & 7.8 & 13.8 & 19.7 & 13.8\\
% \hline
% C1 & CTC & 5.0 & 5.4 & 11.7 & 11.1 & 7.5 & 12.4 & 18.2 & 12.7\\


\toprule
\end{tabular}
}
% \vspace{-0.6cm}
\end{table}


==> tables/t2.tex <==

\begin{table}[h]
\centering

\caption{
WER (\%) of SACTC in MTASR.
"dec." stands for decoding.
}
\vspace{-8pt}
\label{tab:t2}
\scalebox{0.8}{
\renewcommand{\arraystretch}{1.3} % line hight
\begin{tabular}{l|l|cc|cc|cccc}
\bottomrule

\multirow{3}{*}{\textbf{ID}} & \makecell[c]{\multirow{3}{*}{\textbf{System}}}  &\multicolumn{2}{c|}{\textbf{Librispeech}} &\multicolumn{6}{c}{\textbf{LibrispeechMix-2mix}} \\
 \cline{3-4} \cline{5-10} 
& & \multirow{2}{*}{\textbf{dev}} & \multirow{2}{*}{\textbf{test}} & \multirow{2}{*}{\textbf{Dev}} & \multirow{2}{*}{\shortstack{\textbf{Test}\\(Overall)}}& \multicolumn{4}{c}{\textbf{Test} (Conditional)} \\
\cline{7-10}
% & & & & & & \textbf{(0, 20]} & \textbf{(20, 50]} & \textbf{(50, 100]} & \textbf{Average} \\
& & & & & & low & mid & high & OA-WER \\
% & & & & & & low & median & high & OA-WER \\
\noalign{\hrule height 0.9pt}
A1 & SOT & 4.1 & 4.6 & 7.9 & 9.2 & 9.0 & \hl{8.0} & 12.8 & 9.9 \\
\hline
C1 & SOT+CTC & 4.3 & 4.5 & 8.4  & 8.8 & 7.1 & 9.0  & 13.1 & 9.7\\
\hline
D1 & SOT+SACTC & 3.9 & \hl{4.1} & 8.2 & \hl{8.0} & \hl{6.0} & 8.4 & 12.8 & \hl{9.1} \\
D2 & \, $\hookrightarrow$ AED only dec. & 4.0 & 4.5 & 8.4 & 8.8 & 8.2 & \hl{8.0} & \hl{12.3} & 9.5\\
D3 & \, $\hookrightarrow$ CTC only dec. & 5.5 & 5.8 & 12.5 & 11.9 & 8.1 & 13.1 & 19.9 & 13.7\\



\toprule
\end{tabular}
}
\vspace{-14pt}
\end{table}


==> tables/t4.tex <==

\begin{table}[h]
\centering

\caption{
WER (\%) of sole SACTC with different risk factors (RF).
}
\vspace{-8pt}
\label{tab:t4}
\scalebox{0.8}{
\renewcommand{\arraystretch}{1.3} % line hight
\begin{tabular}{l|l|cc|cc|cccc}
\bottomrule

\multirow{3}{*}{\textbf{ID}} & \makecell[c]{\multirow{3}{*}{\textbf{System}}}  &\multicolumn{2}{c|}{\textbf{Librispeech}} &\multicolumn{6}{c}{\textbf{LibrispeechMix-2mix}} \\
 \cline{3-4} \cline{5-10} 
& & \multirow{2}{*}{\textbf{dev}} & \multirow{2}{*}{\textbf{test}} & \multirow{2}{*}{\textbf{Dev}} & \multirow{2}{*}{\shortstack{\textbf{Test}\\(Overall)}}& \multicolumn{4}{c}{\textbf{Test} (Conditional)} \\
\cline{7-10}
% & & & & & & \textbf{(0, 20]} & \textbf{(20, 50]} & \textbf{(50, 100]} & \textbf{Average} \\
& & & & & & low & mid & high & OA-WER \\
% & & & & & & low & median & high & OA-WER \\
\noalign{\hrule height 0.9pt}
B1 & CTC & 5.0 & 5.4 & 11.7 & 11.1 & 7.5 & 12.4 & 18.2 & 12.7\\
\hline
G1 &  SACTC RF=5 & 5.3 & 5.6 & 12.9 & 12.2 & 8.0 & 13.7 & 20.0 & 13.9\\
G2 &  SACTC RF=10 & 5.3 & 5.5 & 12.2 & 11.7 & 7.8 & 13.2 & 18.9& 13.3\\
G3 &  SACTC RF=15 & 5.4 & 5.6 & 13.5 & 12.3 & 8.0 & 13.9 & 20.8 & 14.2\\
G4 &  SACTC RF=20 & 5.4 & 5.6 & 12.6 & 11.7 & 7.8 & 13.2 & 19.0 & 13.3\\



\toprule
\end{tabular}
}
\vspace{-0.6cm}
\end{table}

